Data Interpreter: An LLM Agent For Data Science

Large Language Model (LLM)-based agents have shown effectiveness across many applications. However, their use in data science scenarios requiring solving long-term interconnected tasks, dynamic data adjustments and domain expertise remains challenging. Previous approaches primarily focus on individual tasks, making it difficult to assess the complete data science workflow. Moreover, they struggle to handle real-time changes in intermediate data and fail to adapt dynamically to evolving task dependencies inherent to data science problems. In this paper, we present Data Interpreter, an LLM-based agent designed to automatically solve various data science problems end-to-end. Our Data Interpreter incorporates two key modules: 1) Hierarchical Graph Modeling, which breaks down complex problems into manageable subproblems, enabling dynamic node generation and graph optimization; and 2) Programmable Node Generation, a technique that refines and verifies each subproblem to iteratively improve code generation results and robustness. Extensive experiments consistently demonstrate the superiority of Data Interpreter. On InfiAgent-DABench, it achieves a 25% performance boost, raising accuracy from 75.9% to 94.9%. For machine learning and open-ended tasks, it improves performance from 88% to 95%, and from 60% to 97%, respectively. Moreover, on the MATH dataset, Data Interpreter achieves remarkable performance with a 26% improvement compared to state-of-the-art baselines. The code is available at https://github.com/geekan/MetaGPT.

==> files/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and the introduction highlight the contribution of our paper in solving data science problems utilizing hierarchical graphs and programmable node generation, enabling a programmatic and structured approach to tackle complex tasks. Our framework iteratively optimizes the graph structure with real-time feedback, ensuring continuous refinement and accuracy in dynamic environments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations of the work in the~\Cref{limitations} .%\justificationTODO{
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In \Cref{subsec:hgm}, we use mathematical formalism to clearly and intuitively explain the problem without introducing new theories or hypotheses. This approach helps us define the problem and establish a strong foundation for our subsequent analysis and methodology development.%我们在Setion 3.1 里使用数学形式来直观的说明待解决的问题，没有单独提出新的理论和假设。} %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided the required information in the~\Cref{main:experiments} and~\Cref{appendix:exp-datasets}(see the details in experiments setup) to reproduce the experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: For the ML-Benchmark and Open-ended task benchmarks, as described in \Cref{main:experiments}, we have included the dataset folders in anonymous zip files, as well as the scripts needed to run the experiments. The MATH dataset is open-source, and we also provide the script for running the experiment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the experimental setting details in \Cref{subsec:expsetup}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Although we do not provided the error bars, but we calculate the average and std results, which are provided in~\Cref{tab:ml-score,tab:open-ended-task-score}.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As our framework is mainly focus on exploring the capabilities of LLM-based agents in addressing data science problems, we opt not to fine-tune the LLM. Instead, we leverage OpenAI's API. We use the GPT-4-Turbo (gpt-4-1106-preview) for our method and the baselines.
    %\justificationTODO{% 在附录说明所需的运行环境，minimum 的cpu/memory资源，网络环境正常如果需要使用OpenAI的模型接口}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the NeurIPS Code of Ethics and keep code submissions anonymous.
    %\justificationTODO{%我们已阅读且保持提交代码的匿名性}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the potential positive and negative societal impacts in \Cref{broader impacts}.
    %\justificationTODO{}
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We only use dataset from scientific questions and GPT-4, and will not release the new data and models. We can convert to a more secure LLM without additional cost.
    % \justificationTODO{ %DI提高了LLM解决问题的应用场景，考虑接入有safety polcy的LLMs 可以避免high risk}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use the CC-BY 4.0 license.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide a README file in the anonymous zip files provided, regarding the use of code and the use of data sets.
    % \justificationTODO{% 我们在提供的anonymized zip files里说明提供了Readme，关于代码的使用和数据集的使用}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not include human subjects. %\justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> tables/DABench_performance.tex <==
\begin{table*}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Performance comparisons on DABench.} 
This figure reports the comprehensive score of each method. "xagent", "autogent", and "Data Interpreter" represent different methods, while "GPT-4-0613" and "GPT-4o" represent different LLMs.
}
% \vspace{-0.4cm}
\renewcommand\tabcolsep{5.9pt}
\renewcommand\arraystretch{1.2}
\small
\centering
\begin{tabular}{l|cccccc}
\hline

\hline

\hline

\hline
\multicolumn{1}{l|}{Method} & \multicolumn{1}{c}{XAgent} & \multicolumn{1}{c}{AutoGen} & \multicolumn{1}{c}{Data Interpreter} & \multicolumn{1}{c}{}
& \multicolumn{1}{c}{Data Interpreter} & \multicolumn{1}{c}{}
\\
\midrule
\multicolumn{1}{l|}{LLM} & \multicolumn{1}{c}{GPT-4-0613} & \multicolumn{1}{c}{GPT-4-0613} & \multicolumn{1}{c}{GPT-4-0613}
 & \multicolumn{1}{c}{GPT-4-0613} & \multicolumn{1}{c}{GPT-4o} & \multicolumn{1}{c}{GPT-4o} 
\\
\midrule
\multicolumn{1}{l|}{Score} & \multicolumn{1}{c}{47.52} & \multicolumn{1}{c}{71.48} & \multicolumn{1}{c}{73.55}
 & \multicolumn{1}{c}{78.99} & \multicolumn{1}{c}{\textbf{94.93}} & \multicolumn{1}{c}{75.92} 
\\
\hline

\hline

\hline

\hline
\end{tabular}
    % }
    \label{tab:dabench-score}
\end{table*}


==> tables/ablation_ml.tex <==
% \begin{table*}[t]
% \tablestyle{1.8pt}{1.05}
% \caption{
% \textbf{Ablation on core modules.} Evaluated on ML-Benchmark. ``ICR", ``SCTP", and ``SVPC" represent ``ICR - Identifying age-related conditions", ``Santander customer transaction prediction", and ``Santander value prediction challenge", respectively. ``Avg." denotes ``Average".
% }

% \renewcommand\tabcolsep{4.8pt}
% \renewcommand\arraystretch{1.2}
% \small
% \centering
% \begin{tabular}{cccc|ccccc}
% \hline

% \hline

% \hline

% \hline
% \multicolumn{1}{c}{Code execution} & \multicolumn{1}{c}{Plan strategy} & \multicolumn{1}{c}{Reflective analysis} &\multicolumn{1}{c|}{Tool} & \multicolumn{1}{c}{House Prices} & \multicolumn{1}{c}{SCTP} & \multicolumn{1}{c}{SVPC} &\multicolumn{1}{c}{ICR} & \multicolumn{1}{|c}{Avg.} \\
% \midrule
% \multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{Simple} & \multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.50} & \multicolumn{1}{c}{0.17} & \multicolumn{1}{c}{0.66} & \multicolumn{1}{c}{0.66} & \multicolumn{1}{|c}{0.37} \\

% \multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{Simple} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.79} & \multicolumn{1}{c}{0.83} & \multicolumn{1}{c}{0.86} & \multicolumn{1}{|c}{0.83} \\

% \multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{Hierarchical} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.74} & \multicolumn{1}{c}{0.84} & \multicolumn{1}{|c}{0.86} \\

% \rowcolor[gray]{.9}
% \multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{Hierarchical} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{c}{\textbf{0.94}} & \multicolumn{1}{c}{\textbf{0.98}} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{|c}{\textbf{0.96}} \\
% \hline

% \hline

% \hline

% \hline
% \end{tabular}
% \label{tab:ml-score-abl}
% \end{table*}

\begin{table*}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on core modules.} Evaluated with comprehensive score on ML-Benchmark. `IGO' stands for Iterative Graph Optimization, and `PNG' denotes Programmable Node Generation. ``ICR", ``SCTP'', and ``SVPC'' represent ``ICR - Identifying age-related conditions'', ``Santander customer transaction prediction'', and ``Santander value prediction challenge'', respectively.
}
\renewcommand\tabcolsep{9.2pt}
\renewcommand\arraystretch{1.2}
\small
\centering
\begin{tabular}{cccc|cccc}
\hline

\hline

\hline

\hline
\multicolumn{1}{c}{Code execution} & \multicolumn{1}{c}{IGO} &\multicolumn{1}{c|}{PNG} & \multicolumn{1}{c}{House Prices} & \multicolumn{1}{c}{SCTP} & \multicolumn{1}{c}{SVPC} &\multicolumn{1}{c}{ICR} & \multicolumn{1}{|c}{Avg.} \\
\midrule
\multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.51} & \multicolumn{1}{c}{0.17} & \multicolumn{1}{c}{0.66} & \multicolumn{1}{c}{0.17} & \multicolumn{1}{|c}{0.37} \\

% \multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{Simple} & \multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.79} & \multicolumn{1}{c}{0.83} & \multicolumn{1}{c}{0.86} & \multicolumn{1}{|c}{0.83} \\

\multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{c}{0.91} & \multicolumn{1}{c}{0.80} & \multicolumn{1}{c}{0.74} & \multicolumn{1}{|c}{0.85} \\

\rowcolor[gray]{.9}
\multicolumn{1}{c}{\checkmark} &\multicolumn{1}{c}{\checkmark} & \multicolumn{1}{c|}{\checkmark} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{c}{\textbf{0.95}} & \multicolumn{1}{c}{\textbf{0.89}} & \multicolumn{1}{c}{\textbf{0.96}} & \multicolumn{1}{|c}{\textbf{0.94}} \\
\hline

\hline

\hline

\hline
\end{tabular}
\label{tab:ml-score-abl}
\end{table*}

==> tables/algo_graph_optimization.tex <==
% iterative graph optimization

\begin{algorithm}
\caption{Iterative Graph Optimization}
\label{alg:conciseIterativeGraphOptimization}
\begin{algorithmic}[1]
  
\While{tasks remain}
    \For{each task $\texttt{p}_i$ in action graph $\mathcal{G}\left( \{\texttt{p}_i(x)\}_{i=1}^{n}, \mathcal{R} \right)$ in topological order}  
        \State Execute task code and mark as ``Success'' or ``Failure''  
        \If{task fails or human edits}
            \State Debug task $\texttt{p}_i$ with LLMs or refine with human-in-the-loop  
            \State Regenerate task graph $\mathcal{G}$ and update the graph with prefix matching
        \EndIf  
    \EndFor  
\EndWhile
\State \textbf{return} Updated graph
  
\end{algorithmic}  
\end{algorithm} 

==> tables/exp-tables.tex <==
\begin{table}[h]
\centering
\renewcommand\tabcolsep{10pt}
\renewcommand\arraystretch{1.2}
    \caption{The scoring schema for completion rate computation.}
    % \resizebox{0.45\textwidth}{!}{%
\begin{tabular}{l|c}
\hline

\hline

\hline

\hline
\textbf{Status} & \textbf{Score} \\
\midrule
Missing & 0 \\
% \hline
Fail & 0 \\
% \hline
Success - Non-Compliant & 1 \\
% \hline
Success - Compliant & 2 \\
% \hline
Optional Step & Not involved in scoring \\
% \hline
\hline

\hline

\hline

\hline
\end{tabular}%
    % }
    \label{tab:ml-step-status-transposed}
\end{table}



==> tables/exprience_performance.tex <==
\begin{table}[t]
\tablestyle{1.8pt}{1.05}
\caption{
\textbf{Ablation on experience pool size.} 
% We assess the task efficiency by averaging the number of debugging attempts (NDA) required and the cost for completing the task, exclude the experience retrieval and usage. The mean of multiple attempts is taken. Lower values indicate better performance.
We evaluate the efficiency of completing tasks by taking the average of the number of debugging attempts (NDA) required and the total cost, excluding experience retrieval and usage. We take the mean of multiple attempts to arrive at the final value. Lower values indicate better performance. ``Avg." and ``Std." denote ``Average" and ``Standard deviation", respectively.
}
% \vspace{-0.4cm}
\renewcommand\tabcolsep{6.1pt}
\renewcommand\arraystretch{1.2}
\small
\centering
    % \resizebox{0.8\textwidth}{!}{%
\begin{tabular}{l|ccccccc}
\hline

\hline

\hline

\hline
\multicolumn{1}{l|}{Experience pool size} & \multicolumn{2}{c}{size=0} & 
\multicolumn{2}{c}{size=80} & \multicolumn{2}{>{\columncolor[gray]{.9}}c}{size=200} \\
\multicolumn{1}{l|}{Metric} & \multicolumn{1}{c}{NDA} & \multicolumn{1}{c}{Cost (\$)} & \multicolumn{1}{c}{NDA} & \multicolumn{1}{c}{Cost (\$)} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{NDA} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{Cost (\$)} \\ 

\midrule
\multicolumn{1}{l|}{WSC} & \multicolumn{1}{c}{1.50} & \multicolumn{1}{c}{0.69} &\multicolumn{1}{c}{0.80} &\multicolumn{1}{c}{0.33} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.40}} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.29}} \\

\multicolumn{1}{l|}{ER} & \multicolumn{1}{c}{1.50} & \multicolumn{1}{c}{0.81} & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{0.27} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0}} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.13}} \\

\multicolumn{1}{l|}{Titanic} & \multicolumn{1}{c}{1.40} & \multicolumn{1}{c}{0.65} & \multicolumn{1}{c}{0.40} & \multicolumn{1}{c}{0.35} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.40}} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.31}} \\

\multicolumn{1}{l|}{House Prices} & \multicolumn{1}{c}{1.60} & \multicolumn{1}{c}{1.01} & \multicolumn{1}{c}{0.60} & \multicolumn{1}{c}{0.15} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.40}} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.15}} \\

\multicolumn{1}{l|}{ICR} & \multicolumn{1}{c}{1.40}& \multicolumn{1}{c}{0.85} & \multicolumn{1}{c}{0.60} & \multicolumn{1}{c}{0.44} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.40}} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.37}} \\

\midrule
\multicolumn{1}{l|}{Avg. / Std.} & \multicolumn{1}{c}{1.48 / 0.08} & \multicolumn{1}{c}{0.80 / 0.14} & \multicolumn{1}{c}{0.53 / 0.21} & \multicolumn{1}{c}{0.31 / 0.11} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.32} / 0.18} & \multicolumn{1}{>{\columncolor[gray]{.9}}c}{\textbf{0.24} / 0.10} \\
\hline

\hline

\hline

\hline
\end{tabular}
    % }
    \label{tab:ml-exp}
\end{table}

% \begin{table*}[t]
% \tablestyle{1.8pt}{1.05}
% \caption{
% \textbf{Ablation on experience pool size.} We evaluate the efficiency of task completion for open-ended tasks. Lower is better.
% }
% % \vspace{-0.4cm}
% \renewcommand\tabcolsep{15pt}
% \renewcommand\arraystretch{1.2}
% \small
% \centering
%     % \resizebox{0.8\textwidth}{!}{%
% \begin{tabular}{l|ccccc|c}
% \hline

% \hline

% \hline

% \hline
% \multicolumn{1}{c|}{Experience pool size} & \multicolumn{1}{c}{Web search and crawling} & 
% \multicolumn{1}{l}{Email reply} & \multicolumn{1}{c}{Titanic} & \multicolumn{1}{c}{House Prices} & \multicolumn{1}{|c}{Mean} \\
% \midrule
% \multicolumn{1}{l|}{0} & \multicolumn{1}{c}{1.50} & \multicolumn{1}{c}{1.50} & \multicolumn{1}{c}{1.40} & \multicolumn{1}{c}{1.40} & \multicolumn{1}{|c}{1.50}\\
% \multicolumn{1}{l|}{80} & \multicolumn{1}{c}{0.25} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{0.40} & \multicolumn{1}{c}{1.00} & \multicolumn{1}{|c}{0.36}\\
% \multicolumn{1}{l|}{200} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{0}} & \multicolumn{1}{c}{\textbf{0.20}} & \multicolumn{1}{c}{\textbf{0.60}} & \multicolumn{1}{|c}{\textbf{0.10}}\\
% % \midrule
% \hline

% \hline

% \hline

% \hline
% \end{tabular}
%     % }
%     \label{tab:exp-performance}
% \end{table*}

